User Collusion Avoidance Scheme for Privacy-Preserving Decentralized Key-Policy Attribute-Based Encryption -- Full Version

Recent trend towards cloud computing paradigm, smart devices and 4G wireless technologies has enabled seamless data sharing among users. Cloud computing environment is distributed and untrusted, hence data owners have to encrypt their data to enforce data confidentiality. The data confidentiality in a distributed environment can be achieved by using attribute-based encryption technique. Decentralized attribute-based encryption technique is a variant of multiple authority based attribute-based encryption whereby any attribute authority can independently join and leave the system without collaborating with the existing attribute authorities. In this paper, we propose a privacy-preserving decentralized key-policy attribute-based encryption scheme. The scheme preserves the user privacy when users interact with multiple authorities to obtain decryption keys while mitigating the well-known user collusion security vulnerability. We showed that our scheme relies on decisional bilinear Diffie-Hellman standard complexity assumption in contrast to the previous nonstandard complexity assumptions such as $q-$decisional Diffie-Hellman inversion.

==> DKP-ABE-Algo-1.tex <==
\begin{figure}\small
\setlength{\unitlength}{0.2in} % selecting unit length
\centering % used for centering Figure
\framebox{
\parbox[t][9.6cm]{8cm}{
%\vspace{0.5cm}
\textbf{Global Setup} $\mathcal{(GS)-}$ Same as the original.\\
\textbf{AAs Setup} $\mathcal{(AS)-}$ The initial setup is same as the original. We consider more generic tree access structure. Hence we replace the threshold access structure requirement into tree based as follows: $A_k$ specify $m_k$ as  minimum number of attributes required to satisfy the access structure ( $m_k \leq n_k$).\\
\ \\
\textbf{Key Generation} $\mathcal{(KG)-}$  Attribute set of user is $\tilde{A}_u$: $\tilde{A}_u\cap \tilde{A}_k=\tilde{A}_u^k ~\forall ~k$.
    $A_k$ generates $r_{k,u} \in _{R}  \mathbb{Z}_{p}$ and  polynomial $q_x$ for each node $x$ (including the leaves) $\mathbb{T}$.
     For each node $x$, the degree $d_x$ of the polynomial $q_x$ is $d_x = k_x - 1$  where $k_x$ --  threshold value of that node.
   Now, for the root node $r$, set $q_r(0) = r_{k,u}$.
For any other node $x$, set $q_x(0) = q_{parent(x)}(index(x))$.
 Now decryption keys for the user $u$ is generated as follows:
    $D = D_{k,u}=g^{-\alpha_k}h^{\frac{\beta_k}{r_{k,u}+u}}h_1^{\frac{r_{k,u}}{\beta_k+u}}, D_{k,u}^1=h^{\frac{1}{r_{k,u}+u}}, D_{k,u}^j=h_1^{\frac{q_{a_{k,j}}(0)}{(\beta_k+u)t_{k,j}}}, \forall a_{k,j} \in \tilde{A}_u^k$.\\
    \ \\
\textbf{Encryption} $\mathcal{(E)-}$ This exactly same as the original scheme.\\
\textbf{Decryption} $\mathcal{(D)-}$ In order to decrypt $C$, the user $u$, computes $X,~Y$ and $S_k$ as follows:   $X = \prod\limits_{k \in I_C} e\left(C_2,D_{k,u}\right),~Y =  e\left(C_3,D_{k,u}^1\right) \textrm{and}~S_k=\prod\limits_{a_{k,j} \in A_m^k}e\left(C_{k,j}, D_{k,u}^j\right)^{\Delta_{a_{k,j} ,\tilde{A}_m^j}(0)}$.  User then decrypts the message $m$ as follows: $m=\frac{C_1X}{Y\prod\limits_{k \in I_C}S_k}$.
}}
\caption{The proposed decentralized KP-ABE scheme. This shows the difference between the original and the proposed algorithm.}
\label{proposed algorithm}
\end{figure} 

==> DKP-ABE-Algo-Original.tex <==
\begin{figure}\small
\setlength{\unitlength}{0.2in} % selecting unit length
\centering % used for centering Figure
\framebox{
\parbox[t][13.5cm]{8cm}{
%\vspace{0.5cm}
\textbf{Global Setup} $\mathcal{(GS)-}$ For a given security parameter $\lambda$, $\mathcal{GS}$ generates the bilinear groups $\mathbb{G}_1$ and $\mathbb{G}_2$ with prime order $p$ as follows: ${\{\mathbb{G}_{1}, \mathbb{G}_{2}\} \leftarrow \mathcal{GS}(1^{\lambda })}$. Let $e: \mathbb{G}_{1}\times\mathbb{G}_{1}\longrightarrow\mathbb{G}_{2}$ be a bilinear map and $g$, $h$ and $h_1$ be the generators of $\mathbb{G}_{1}$. There are $N$ number of authorities $\{A_1,\ldots,A_N\}$: $A_k$ monitors $n_k$ attributes i.e. $\tilde{A}_k=\{a_{k,1}\ldots,a_{k,n_k}\}, \forall k$.\\
\ \\
\textbf{AAs Setup} $\mathcal{(AS)-}$ Security parameters of $A_k$:
   $SK_k = \left\{ \alpha_{k}, \beta_k,~ \textrm{and}~ [t_{k,1},\ldots,t_{k,n_k}]\right\} ~\underleftarrow{~~R~~} \mathbb{Z}_{p}, \forall k$. Public parameters of $A_k$: $PK_k$ = \{$Y_{k} = e(g, g)^{\alpha_k}$, $Z_{k} = g^{\beta_k}$, and $[T_{k,1}=g^{t_{k,1}},\ldots,T_{k,n_k}=g^{t_{k,n_k}}]\}$, $\forall$ $k$. Each $A_k$ specifies an  $(k_k, n_k)$ threshold access structure where $k_k \leq n_k$.\\
   \ \\
\textbf{Key Generation} $\mathcal{(KG)-}$    Collision-Resistant Hash Function $H: \left \{ 0,1 \right \}^{*} \rightarrow \mathbb{Z}_{p}$ to generate  $u$ from the user global identity.     Attribute set of user is $\tilde{A}_u$: $\tilde{A}_u\cap \tilde{A}_k=\tilde{A}_u^k ~\forall ~k$.
    $A_k$ generates $r_{k,u} \in _{R}  \mathbb{Z}_{p}$ and  $d_k = k_k - 1$ degree polynomial $q_k$ where $k_k$ --  threshold value of that node.
   with $q_k(0) = r_{k,u}$. Now decryption keys for the user $u$ is generated as follows:
    $D = D_{k,u}=g^{\alpha_k}h^{r_{k,u}}h_1^{u\beta_k}, D_{k,j}=h^{\frac{q_k(a_{k,j})}{t_{k,j}}}, \forall a_{k,j} \in \tilde{A}_u^k$.\\
    \ \\
\textbf{Encryption} $\mathcal{(E)-}$ Attribute set for the message $m$ is $\tilde{A}_m$: $\tilde{A}_m\cap \tilde{A}_k=\tilde{A}_m^k, \forall k$, i.e. $\tilde{A}_m= \{ \tilde{A}_m^1,\ldots,\tilde{A}_m^k,\ldots,\tilde{A}_m^N \}$.Data owner of message $m$ randomly chooses $s \in _{R} \mathbb{Z}_{p}$, and output the ciphertext as follows:\\ $C = C_1 = m.\prod\limits_{k \in I_C}e(g, g)^{\alpha_ks}, C_2= g^{s}, C_3=\prod\limits_{k \in I_C}g^{\beta_ks} \textrm{and} \left \{ C_{k,j} = T_{k,j}^{s} \right \}_{\forall k\in I_{C}, a_{k,j} \in \tilde{A}_m^j}$ where $I_c$ denotes the index set of the authorities.\\
\ \\
\textbf{Decryption} $\mathcal{(D)-}$ In order to decrypt $C$, the user $u$, computes $X,~Y$ and $S_k$ as follows:   $X = \prod\limits_{k \in I_C} e\left(C_2,D_{k,u}\right),~Y =  e\left(C_3,h_1^u\right) \textrm{and}~S_k=\prod\limits_{a_{k,j} \in A_m^k}e\left(C_{k,j}, D_{k,j}\right)^{\Delta_{a_{k,j} ,\tilde{A}_m^j}(0)}$.  User then decrypts the message $m$ as follows: $m=\frac{C_1Y\prod\limits_{k \in I_C}S_k}{X}$.}}
\caption{The original decentralized key-policy attribute-based encryption scheme \cite{main1}.}
\label{main algorithm}
\end{figure} 
